Oryx: a Scalable Sequence Model for Many-Agent Coordination in Offline MARL

A key challenge in offline multi-agent reinforcement learning (MARL) is achieving effective many-agent multi-step coordination in complex environments. In this work, we propose Oryx, a novel algorithm for offline cooperative MARL to directly address this challenge. Oryx adapts the recently proposed retention-based architecture Sable and combines it with a sequential form of implicit constraint Q-learning (ICQ), to develop a novel offline autoregressive policy update scheme. This allows Oryx to solve complex coordination challenges while maintaining temporal coherence over long trajectories. We evaluate Oryx across a diverse set of benchmarks from prior works -- SMAC, RWARE, and Multi-Agent MuJoCo -- covering tasks of both discrete and continuous control, varying in scale and difficulty. Oryx achieves state-of-the-art performance on more than 80% of the 65 tested datasets, outperforming prior offline MARL methods and demonstrating robust generalisation across domains with many agents and long horizons. Finally, we introduce new datasets to push the limits of many-agent coordination in offline MARL, and demonstrate Oryx's superior ability to scale effectively in such settings.

==> tables/cfcql_mpe.tex <==
\begin{table}[h!]
    \centering
    \caption{Results on Multi-agent Particle Environment datasets from OMAR. Results from CFCQL.}
    \begin{adjustbox}{max width=1.\textwidth}
    \begin{tabular}{l|cccc|cccc|cccc}
        \toprule
        \textbf{Algorithm} & \multicolumn{4}{c}{\textbf{CN}} & \multicolumn{4}{c}{\textbf{PP}} & \multicolumn{4}{c}{\textbf{World}} \\
        \midrule
        & Random & Med-Rep & Medium & Expert & Random & Med-Rep & Medium & Expert & Random & Med-Rep & Medium & Expert \\
        \midrule
        OMAR & 34.4$\pm$5.3 & 37.9$\pm$12.3 & 47.9$\pm$18.9 & \textbf{114.9$\pm$2.6} & 11.1$\pm$2.8 & 47.1$\pm$15.3 & 66.7$\pm$23.2 & 116.2$\pm$19.8 & 5.9$\pm$5.2 & 42.9$\pm$19.5 & 74.6$\pm$11.5 & 110.4$\pm$25.7 \\
        MACQL & 45.6$\pm$8.7 & 25.5$\pm$5.9 & 14.3$\pm$20.2 & 12.2$\pm$31 & 25.2$\pm$11.5 & 11.9$\pm$9.2 & 55$\pm$43.2 & 108.4$\pm$21.5 & 11.7$\pm$11 & 13.2$\pm$16.2 & 67.4$\pm$48.4 & 99.7$\pm$31 \\
        IQL & 5.5$\pm$1.1 & 10.8$\pm$4.5 & 28.2$\pm$3.9 & 103.7$\pm$2.5 & 1.3$\pm$1.6 & 23.2$\pm$12 & 53.6$\pm$19.9 & 109.3$\pm$10.1 & 2.9$\pm$4.0 & 41.5$\pm$9.5 & 70.5$\pm$15.3 & 107.8$\pm$17.7 \\
        CFCQL & \textbf{62.2$\pm$8.1} & \textbf{52.2$\pm$9.6} & \textbf{65.0$\pm$10.2} & 112$\pm$4 & \textbf{78.5$\pm$15.6} & \textbf{71.1$\pm$6} & \textbf{68.5$\pm$21.8} & \textbf{118.2$\pm$13.1} & \textbf{68$\pm$20.8} & \textbf{73.4$\pm$23.2} & \textbf{93.8$\pm$31.8} & \textbf{119.7$\pm$26.4} \\
        \midrule
        \textbf{Offline Sable} & 0.0$\pm$0.0 & 0.0$\pm$0.0 & 0.0$\pm$0.0 & 0.0$\pm$0.0 & 0.0$\pm$0.0 & 0.0$\pm$0.0 & 0.0$\pm$0.0 & 0.0$\pm$0.0 & 0.0$\pm$0.0 & 0.0$\pm$0.0 & 0.0$\pm$0.0 & 0.0$\pm$0.0 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table}


==> tables/omiga.tex <==
\begin{table}[hbtp]
    \centering
    \caption{Results on SMACv1 datasets from OMIGA~\citet{omiga}. Other Results from OMIGA.}
    \begin{adjustbox}{max width=\textwidth} 
\begin{tabular}{ll|lllll|ll}

Task & Dataset Quality & MABCQ & MACQL & MAICQ & OMAR & OMIGA & IQL+CQL & Offline Sable \\
\midrule
\multirow[t]{3}{*}{2c\_vs\_64zg} & Good & 19.13$\pm$0.27 &  18.48$\pm$0.95* & 18.82$\pm$0.17 & 17.27$\pm$0.78 &  19.15$\pm$0.32* & 19.52$\pm$0.26 & \textbf{19.95$\pm$0.24}\\
 & Medium &  15.58$\pm$0.37* & 12.82$\pm$1.61 &  15.57$\pm$0.61* & 10.20$\pm$0.20 & \textbf{16.03$\pm$0.19} & 14.89$\pm$0.72 & 15.73$\pm$0.51\\
 & Poor &  12.46$\pm$0.18* & 10.83$\pm$0.51 &  12.56$\pm$0.18* & 11.33$\pm$0.50 & \textbf{13.02$\pm$0.66} & 11.03$\pm$0.41 & 10.71$\pm$0.36\\
\cline{1-9}
\multirow[t]{3}{*}{5m\_vs\_6m} & Good & 7.76$\pm$0.15 & 8.08$\pm$0.21 & 7.87$\pm$0.30 & 7.40$\pm$0.63 & 8.25$\pm$0.37 & \textbf{12.36$\pm$1.09} & 11.64$\pm$0.69 \\
 & Medium & 7.58$\pm$0.10 & 7.78$\pm$0.10 & 7.77$\pm$0.30 & 7.08$\pm$0.51 & 7.92$\pm$0.57 & \textbf{12.30$\pm$0.74} & 12.20$\pm$0.72 \\
 & Poor & 7.61$\pm$0.36 & 7.43$\pm$0.10 & 7.26$\pm$0.19 & 7.27$\pm$0.42 & 7.52$\pm$0.21 & 10.20$\pm$0.75 & \textbf{10.85$\pm$0.67} \\
\cline{1-9}
\multirow[t]{3}{*}{6h\_vs\_8z} & Good & 12.19$\pm$0.23 & 10.44$\pm$0.20 & 11.81$\pm$0.12 & 9.85$\pm$0.28 &  12.54$\pm$0.21* & 12.72$\pm$0.44 & \textbf{12.87$\pm$0.36} \\
 & Medium & 11.77$\pm$0.16 & 11.29$\pm$0.29 & 11.13$\pm$0.33 & 10.36$\pm$0.16 & \textbf{12.19$\pm$0.22} &  12.01$\pm$0.42* & 11.97$\pm$0.24\\
 & Poor & 10.84$\pm$0.16 &  10.81$\pm$0.52* & 10.55$\pm$0.10 & 10.63$\pm$0.25 & \textbf{11.31$\pm$0.19} & 10.41$\pm$0.36 & 10.61$\pm$0.19 \\
\cline{1-9}
\multirow[t]{3}{*}{corridor} & Good & 15.24$\pm$1.21 & 5.22$\pm$0.81 & 15.54$\pm$1.12 & 6.74$\pm$0.69 & 15.88$\pm$0.89 & 19.06$\pm$0.81 & \textbf{19.79$\pm$0.5} \\
 & Medium & 10.82$\pm$0.92 & 7.04$\pm$0.66 & 11.30$\pm$1.57 & 7.26$\pm$0.71 & 11.66$\pm$1.30 & 13.44$\pm$1.31 & \textbf{17.50$\pm$0.56} \\
 & Poor & 4.47$\pm$0.94 & 4.08$\pm$0.60 & 4.47$\pm$0.33 & 4.28$\pm$0.49 &  5.61$\pm$0.35* & 6.11$\pm$1.10 & \textbf{10.36$\pm$0.54}\\

\end{tabular}
\end{adjustbox}
    \label{tab:smac_omiga}
\end{table}
